Adversarial Auto-Augment with Label Preservation: A Representation Learning Principle Guided Approach

Data augmentation is a critical contributing factor to the success of deep learning but heavily relies on prior domain knowledge which is not always available. Recent works on automatic data augmentation learn a policy to form a sequence of augmentation operations, which are still pre-defined and restricted to limited options. In this paper, we show that a prior-free autonomous data augmentation's objective can be derived from a representation learning principle that aims to preserve the minimum sufficient information of the labels. Given an example, the objective aims at creating a distant "hard positive example" as the augmentation, while still preserving the original label. We then propose a practical surrogate to the objective that can be optimized efficiently and integrated seamlessly into existing methods for a broad class of machine learning tasks, e.g., supervised, semi-supervised, and noisy-label learning. Unlike previous works, our method does not require training an extra generative model but instead leverages the intermediate layer representations of the end-task model for generating data augmentations. In experiments, we show that our method consistently brings non-trivial improvements to the three aforementioned learning tasks from both efficiency and final performance, either or not combined with strong pre-defined augmentations, e.g., on medical images when domain knowledge is unavailable and the existing augmentation techniques perform poorly. Code is available at: https://github.com/kai-wen-yang/LPA3}{https://github.com/kai-wen-yang/LPA3.

==> a1_preliminary.tex <==

\section{Basics of Information Theory}
Our analyses make frequent use of information theoretical quantities~\cite{cover1991information}.
% entropy
Given a joint distribution $P_{\rv{X},\rv{Y}}$ and its marginal distributions $P_{\rv{X}}$, $P_{\rv{Y}}$, we define their {\em entropy} as $H(\rv{X}, \rv{Y}) = \mathrm{E}_{\rv{X},\rv{Y}}[-\log P(x, y)]$, $H(\rv{X}) = \mathrm{E}_{\rv{X}}[-\log P(x)]$, and $H(\rv{Y}) = \mathrm{E}_{\rv{Y}}[-\log P(y)]$.
% conditional entropy
Furthermore, we define the {conditional entropy} of $\rv{X}$ given $\rv{Y}$ as $H(\rv{X}|\rv{Y}) = \mathrm{E}_{\rv{Y}}[-\log H(\rv{X}|y)] = H(\rv{X}, \rv{Y}) - H(\rv{Y})$. % mutual information
Finally, we define the mutual information between $\rv{X}$ and $\rv{Y}$ as $I(\rv{X} \wedge \rv{Y}) = H(\rv{X}) - H(\rv{X}|\rv{Y}) = H(\rv{X}) + H(\rv{Y}) - H(\rv{X}, \rv{Y})$.


==> archive/s4.5_theory_old.tex <==
\section{Theoretical Interpretation}\label{sec:theory}

\subsection{Problem Setup}

Let $P_{\rvx, \rvy}(\cdot, \cdot)$ be the joint distribution of data \textit{observation} $\rvx$ and \textit{label} $\rvy$, where $\rvx$ is a random vector taking values on $\set{X}$ (e.g. images), and $\rvy$ is a (discrete) random variable taking values on $\set{Y}$. 

We define a nuisance as a random vector $\nuisance$ such that for the joint distribution $P_{\rvx, \rvy}(\cdot, \cdot)$, the observed data point $\rvx$ can be always written as a deterministic function of the label $\rvy$ and a nuisance $\nuisance$, and $\nuisance \indep \rvy$, which is supported by Lemma~\ref{lem:nuisance}.
In other words, $\nuisance$ encodes all the randomness of $\rvx$ given $\rvy$, i.e., $H(\rvx \vert \rvy) = H(\nuisance)$.

\begin{lemma}[Task-nuisance Decomposition, Proposition 2.1 by Achille et al.~\cite{achille2018emergence}]
\label{lem:nuisance}
Given a joint distribution $P_{\rvx,\rvy}$, where $\rvy$ is a discrete random variable, we can always find a random variable $\nuisance$ independent of $\rvy$ 
such that $\rvx=d(\rvy,\nuisance)$, for some deterministic function $d$.
\end{lemma}
We call the function $d$ \textit{data generating function}.
The following two mild assumptions are needed for our main theoretical analysis.

\begin{assumption}
\label{assump:determinstic}
    There exists a deterministic function $\pi: \set{X} \to \set{Y}$, i.e., $H(\rvy|\rvx)=0$.
\end{assumption}
Intuitively, we assume that there exists a perfect classifier that can identify the label $y$ based on the observation $x$ with no error, which is common in practice.

\begin{assumption}
\label{assump:discrete}
    The sample space $\set{X}$ is discrete.
\end{assumption}
In practice, the sample space is an image space with a fixed size, for example, $64\times 64$ pixels with 3 RGB channels. And each pixel in each channel takes integer values from 0 to 255. Therefore, it is natural to make this assumption.

\begin{assumption}
\label{assump:addition}
    The data generation function $d$ introduced in Lemma~\ref{lem:nuisance} can be modeled by the summation of a label-relevant variable and a label-irrelevant variable. That is, there exist functions $h_1$ and $h_2$ such that
    $\rvx = d(\rvy, \nuisance) = h_1(\rvy) + h_2(\nuisance)$.
\end{assumption}
Assumption~\ref{assump:addition} supposes that an observation $x$ can be disentangled as the summation of a label-relevant part and a label-irrelevant part. For example, $h_1(\rvy)$ can be the contour and texture of an object, and $h_2(\nuisance)$ can be the background or the details in the image.

\begin{lemma}
\label{lem:det_nuis}
If Assumption~\ref{assump:determinstic} and Assumption~\ref{assump:addition} hold, then there exists a deterministic function $\rho$ such that $\rho(\rvx)=h_2(\nuisance)$, where $\nuisance$ is the nuisance corresponding to $\rvx$. That is, $H(h_2(\nuisance)|\rvx) = 0$.
\end{lemma}
Lemma~\ref{lem:det_nuis} suggests that the nuisance part can be identified and disentangled from an observation.

\begin{lemma}
\label{lem:vary_nuis}
If Assumption~\ref{assump:determinstic} and Assumption~\ref{assump:addition} hold, then for any $x_1=h_1(y)+h_2(z_1)$ and $x_2=h_1(y)+h_2(z_2)$, we have $\pi(x_1)=\pi(x_2)=y$.
\end{lemma}
Lemma~\ref{lem:vary_nuis} shows that changing nuisance does not change the class of an observation.

\subsection{Minimal Sufficient Representation}

\begin{definition}[Minimal Sufficient Representation]
For a Markov chain $\rvy \to \rvx \to \rep$, we say that a representation $\rep$ of $\rvx$ is sufficient for $\rvy$ if $I( \rep \wedge \rvy ) = I( \rvx \wedge \rvy )$; $\rep$ is minimal if $I( \rep \wedge \rvx ) \leq I( \tilde{\rep} \wedge \rvx )$ for all sufficient $\tilde{\rep}$'s.
\end{definition}

\begin{definition}[$\epsilon$-Minimal Sufficient Representation]
For a Markov chain $\rvy \to \rvx \to \rep$, we say that a representation $\rep$ is minimal sufficient if $\rep$ is sufficient and $I( \rep \wedge \rvx ) \leq I( \tilde{\rep} \wedge \rvx ) + \epsilon$ for all sufficient $\tilde{\rep}$'s.
\end{definition}

% We propose to optimize the following problem
% \begin{equation}
% \label{eq:obj}
% \begin{aligned}
%     & \max_{\rv{Z}^\prime} & & I(\rv{Z}^\prime \wedge \rv{X}^\prime) \\
%     & s.t. & & I(\rv{Z}^\prime \wedge \rv{A}) = 0 
% \end{aligned}
% \end{equation}

\begin{theorem}
\label{thm:min_suff_eps}
    Consider label variable $\rvy$, observation variable $\rvx$ and nuisance variable $\nuisance$ satisfying Assumption~\ref{assump:determinstic}, \ref{assump:discrete} and \ref{assump:addition}.
    Let $\rvx^\prime = \rvx - D(\nuisance) + D(\nuisance^\prime)$, where $\nuisance^\prime$ is independent and identically distributed as $\nuisance$.
    % Consider a Markov field $(\rvy, \nuisance) \to \rvx$, $(\rvx, \rva) \to \rvxa$.
    Let $\rep^*$ be a solution to 
    $$\mathrm{argmax}_{\rep} I(\rep \wedge \rvxa) \text{ subject to } I(\rep \wedge \nuisance^\prime) = 0.$$ 
    Then, $\rep^*$ is a $\epsilon$-minimal sufficient representation of $\rvx$ for label $\rvy$ if the following conditions hold:\\
    (a) $I(\rvxa \wedge \rvy) = I(\rvx \wedge \rvy)$ ($\rvxa$ is an in-class augmentation) and \\
    (b) $I(\rvxa \wedge \nuisance) \leq \epsilon$ ($\rvxa$ does not remain much information about $\nuisance$).
\end{theorem}
\paragraph{Remarks.} 
(1) If $D=h_2$, then condition (a) and (b) are perfectly satisfied with $\epsilon=0$, and thus $\rep^*$ is a minimal-sufficient representation of $x$.



==> archive/s4_method_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Class-Disentangled Adversarial Data Augmentation for Semi-Supervised Learning}

Find a data augmentation $X'$ by adding adversarial perturbation to $X$, i.e., $X'=X+\delta$.

\begin{equation}
\begin{aligned} 
&\min_{X'} I(X';N)\\ \label{original}
&\begin{array}{r@{\quad}r@{}l@{\quad}l}
s.t. &I(X';Y)=I(X;Y)
\end{array}
\end{aligned}
\end{equation}

Since $I(X';X)=I(X';N)+I(X';Y)$, Eq.~(\ref{original}) equals to:

\begin{equation}
\begin{aligned} 
&\min_{X'} I(X';X)\\ \label{transform}
&\begin{array}{r@{\quad}r@{}l@{\quad}l}
s.t. &I(X';Y)=I(X;Y)
\end{array}
\end{aligned}
\end{equation}

The Lagrangian relaxation for Eq.~(\ref{transform}) with a fixed penalty parameter $\gamma>0$ :

\begin{equation}
\begin{aligned} 
&\min_{X'} I(X';X)-\gamma I(X';Y)\\
\end{aligned}
\end{equation}

where $-I(X';Y)$ can be measured by cross entropy loss $L_{\rm CE}(X',Y;\theta)$. As to the first term, we have $I(X';X)=H(X)-H(X|X')$ where $H(X)$ does not contain $X'$, thus we only need to calculate $-H(X|X')$.

\begin{equation}
-H(X|X')=\mathbb{E}[{\rm log}P_{\phi}(X|X')]
\end{equation}

\subsection{Relax the class-preserving constraint}
Turn the original class-preserving constraint $I(X';Y)=I(X;Y)$ into $F(X';\theta)=F(X;\theta)$.

Then the objective is:

\begin{equation}
\begin{aligned} 
&\min_{X'} I(X';X)\\ \label{transform}
&\mathrm{ s.t.}~I(X;Y)-I(X';Y)\leq \sigma
\end{aligned}
\end{equation}

Solution:

\begin{equation}
\begin{aligned} 
&\min_{X'} -\sum_{l=1}^{N-1}\| F_l(X';\theta)-F_l(X;\theta) \|_2\\ \label{transform}
&\mathrm{s.t.}~ F(X_i;\theta)[Y]-F(X_i';\theta)[Y]  \leq \sigma
\end{aligned}
\end{equation}

Lagrangian:
\begin{equation}
\min_{X'} -\sum_{l=1}^{N-1}\| F_l(X';\theta)-F_l(X;\theta) \|_2+\gamma \max(0, F(X_i;\theta)[Y]-F(X_i';\theta)[Y]-\sigma)
\end{equation}


\subsection{Add Negative Samples}
\begin{equation}
\begin{aligned} 
&\max_{X''} I(X'';X)\\ \label{transform}
&\mathrm{ s.t.}~I(X;Y)-I(X'';Y)\geq \sigma_{neg}
\end{aligned}
\end{equation}

Solution:

\begin{equation}
\begin{aligned} 
&\min_{X''} \sum_{l=1}^{N-1}\| F_l(X'';\theta)-F_l(X;\theta) \|_2\\ \label{transform}
&\mathrm{s.t.}~ D_{\rm KL}(\hat{F}(X_i'';\theta)\|\hat{F}(X_i;\theta))\geq \sigma_{neg}
\end{aligned}
\end{equation}


% \begin{figure}[htp]
% \centering
% \includegraphics[scale=0.7]{pipeline2.png}
% \caption{\small Latent space class-disentangled VAE.}
% \label{fig:CDVAE}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Semi-supervised learning}
 Finally we use the adversarially augmented data for semi-supervised learning:

\begin{equation}
\begin{aligned} 
 \min_{\theta}~&\mathbb{E}_{(X,Y)\sim P_L(X, Y)}\left[-Y\log F(X;\theta)\right]+\mathbb{E}_{X\sim P_U(X)}\left[-\mathbb{I}(\max_{i}F(X;\theta)[i]\geq\tau )\hat{F}(X;\theta)^T\log F(s(X);\theta)\right]  \\
 &+\mathbb{E}_{X\sim P_U(X)}\left[-\hat{F}(X;\theta)^T\log F(X';\theta)\right]-\mathbb{E}_{X\sim P_U(X)}\left[-\hat{F}(X;\theta)^T\log F(X'';\theta)\right](\textcolor{red}{Gradient~explosion})
\end{aligned}
\end{equation}

or

\begin{equation}
\begin{aligned} 
 \min_{\theta}~&\mathbb{E}_{(X,Y)\sim P_L(X, Y)}\left[-Y\log F(X;\theta)\right]+\mathbb{E}_{X\sim P_U(X)}\left[-\mathbb{I}(\max_{i}F(X;\theta)[i]\geq\tau )\hat{F}(X;\theta)^T\log F(s(X);\theta)\right] \\
 &+\mathbb{E}_{X\sim P_U(X)}\left[-\hat{F}(X;\theta)^T\log F(X';\theta)\right]+\mathbb{E}_{X\sim P_U(X)}\left[-Y''^T\log F(X'';\theta)\right]
\end{aligned}
\end{equation}

\begin{algorithm}[htb]
\caption{Adaptive epsilon}
\label{alg:Framwork}
\begin{algorithmic}[1]
\REQUIRE ~~\\
   Training dataset (X,Y);\\
   The class preserving margin $\sigma$;\\
   Scheduling parameter $\eta$;\\
   Initial every samples' $\epsilon_i$ with 0;\\
   Perturbation upperbound $\epsilon_{max}$;\\

\ENSURE ~~\\ 
     \FOR{epoch$=1,...,N$}
          \FOR{$i=1,...,B$}
          \STATE $X_i'=s(X_i)+\epsilon_i{\rm sign}(\nabla_{\delta}(\sum_{l}\| F_l(X_i;\theta)-F_l(s(X_i);\theta) \|_2)$ \\
    \IF{$D_{\rm KL}(\hat{F}(X_i';\theta)\|\hat{F}(X_i;\theta))\leq \sigma$}
        \STATE $\epsilon_i$=$\epsilon_i$+$\eta$
    \ELSE
        \STATE $\epsilon_i$=$\epsilon_i$-$\eta$
    \ENDIF
    \STATE $\epsilon_i=\min(\epsilon_i,\epsilon_{max})$
    \STATE Use $X'$ as data augmentation for semi-supervised learning.
    \ENDFOR
    \ENDFOR
\end{algorithmic}
\end{algorithm}


 

==> archive/s5_exp_old.tex <==



\section{Experiments}
\subsection{Semi-supervised Classification}
\begin{itemize}
    \item \textcolor{red}{``FixMatch + ours'' vs FixMatch on CIFAR10 and CIFAR100}
    \item \textcolor{red}{Walk-clock time comparison.}
    \item \textcolor{red}{Ablation study}
    \item other datasets/methods.
    \item other metrics: smoothness, optimizing stabability pick accuracy
\end{itemize}
\subsection{Noise-label classification}
\begin{itemize}
    \item \textcolor{red}{`DivideMix + ours'' vs DivideMix on CIFAR10 and CIFAR100}
\end{itemize}
\subsection{Class-imblanced classification}
\begin{itemize}
    \item \textcolor{red}{`Decoupled + ours'' vs Decoupled on CIFAR10 and CIFAR100}
\end{itemize}


\section{Potential Task}
 \subsection{Knowledge Distillation for data augmentation in Self-supervised Learning}
 We can access a model trained on labeled data.
 
 We use this model to distill knowledge for data augmentation in SSL.
 
 
 
 \section{Semi-supervised Representation Learning}
 Representation learning: do not have classifier.
 
 Semi-supervised learning: do not have representations.
 
 
% \section{Potential Task: Semi-supervised Representation Learning}
% How to learn a good representation with few labeled data?
% Formulation--Contrastive learning + semi-supervised learning:
% \begin{equation}
% \begin{aligned} 
%  \min_{\theta}~&\mathbb{E}_{(X,Y)\sim P_L(X, Y)}\left[-Y\log F(X;\theta)\right]+\mathbb{E}_{X\sim P_U(X)}\left[-\mathbb{I}(\max_{i}F(X;\theta)[i]\geq\tau )\hat{F}(X;\theta)^T\log F(s(X);\theta)\right]
%  \\+&\mathbb{E}_{X\sim P_U(X)}(L_{NCE}) 
% \end{aligned}
% \end{equation}


==> archive/s_reports.tex <==
\section{Meeting Records}
\subsection{2022.4.6}
TODO List:
\begin{itemize}
\item Try hard constraint.
\item Select hard margin samples.
\item Try other loss function to avoid gradient explosion.
\item Try class imblance situation. 
\end{itemize}
\subsection{2022.3.14}
TODO List:
\begin{itemize}
\item Apply time-consistency algorithm to data selection, this may solve the ``forgetting'' problem of DNN.
\item Select 10 sample and draw the trend of epsilon.
\item Select three groups of sample, and draw the trend of epsilon for each group.
\end{itemize}
\subsection{2022.3.1}
TODO List:
\begin{itemize}
\item Ablation study of $\epsilon$, which type of $\epsilon$ is beneficial for the training.
\item Other sensitivity analysis.
\item Think about data selection and how to combine it with our data augmentation.
\end{itemize}
\subsection{2022.2.22}
TODO List:
\begin{itemize}
\item Try PGD, CAT, FPAT.
\item Data selection.
\end{itemize}
\subsection{2022.2.15}
TODO List:
\begin{itemize}
\item Try time-consistency/space-consistency regularization and combine this criteria with the current data augmentation formulation.
\item Train the model for longer epochs.
\end{itemize}
\subsection{2022.2.8}
TODO List:
\begin{itemize}
\item Conduct experiments on STL-10 (CIFAR has been overfitted).
\item Try different values of perturbation norm.
\item Try perceptual distance.
\item Seek other potential tasks, where data augmentation is important, such as class-imbalance and fairness.
\end{itemize}
\subsection{2022.1.5}
TODO List:
\begin{itemize}
\item Check whether batch normalization can solve distribution shift.
\item Check whether mixup can solve distribution shift.
\item Try applying dropout perturbation to different layers.
\item Try adding gaussian noise and match the variance.
\end{itemize}
\subsection{2021.12.21}
TODO List:
\begin{itemize}
\item Check the natural data accuracy of model trained on our data augmentation.
\item Try use dropout, add bounded gaussian noise, or add a $l_2$-norm constraint to generate $z'$
\end{itemize}
\subsection{2021.12.14}
TODO List:
\begin{itemize}
\item Compare the results of with and without class disentanglement 
\item Use more effective generateive model such as NVAE.
\end{itemize}
\subsection{2021.12.7}
TODO List:
\begin{itemize}
\item Visualization: apply the same random $z_N$ to different images belonging to the same class and see if the resulted reconstructions are the same.
\item Visualization: check the reconstruction of random $z_N$ and random $z_Y$.
\item Objective change: add KL divergence between $z_N$ and $\mathcal N(0,1)$.
\item Visualization: use random $z_N$ to generate augmentations and check if the augmentations are diverse within the same class (it might require to tune the weight for the KL divergence term). 
\item Model change: change the classifier $F(\cdot)$ to be a network taking images as its input.
\end{itemize}
\subsection{2021.12.1}
TODO List:
\begin{itemize}
    \item Use small dimension of $z_y$.
    \item Evaluate the method on semi/self-supervised learning.
 \end{itemize}  
\subsection{2021.11.24}
TODO List:
\begin{itemize}
    \item Formulate Yanchao's proposal: use $x$-$x'$+$x''$ as a augmentation, where $x''$ is generated by fixing $y$ and perturbing $n$.
    \item Think about how to directly generate latent augmented feature.
 \end{itemize}  
\subsection{2021.11.10}
TODO List:
\begin{itemize}
    \item Add contrastive learning to data with low confidence, while use pesudo-label to data with high confidence.
    \item Adjust loss weight.
 \end{itemize}  
Potential Solutions:
\begin{itemize}
    \item Prototype: each class compute prototype than force representation belong to the same class to be close to the prototype.
\end{itemize}

\subsection{2021.11.3}
TODO List:
\begin{itemize}
    \item formulation: using pseudo-label instead of representation
    \item part-based disentanglement, i.e., NMF (partition pixel space) \href{https://proceedings.neurips.cc/paper/2000/file/f9d1152547c0bde01830b7e8bd60024c-Paper.pdf}{https://proceedings.neurips.cc/paper/2000/file/f9d1152547c0bde01830b7e8bd60024c-Paper.pdf}
    \item add contrastive loss or supervised contrastive loss
    \item prove the necessity of \textbf{minimal} information
    \item add constraint to $D(z)$ to encourage orthogonality
    \item try only using our data augmentation (wo strong augmentation)
\end{itemize}

Potential Solutions:
\begin{itemize}
    \item deep clustering (for self-supervised learning):\\ \href{https://arxiv.org/pdf/1807.05520.pdf}{https://arxiv.org/pdf/1807.05520.pdf}, \\
    \href{https://arxiv.org/pdf/2006.09882.pdf}{https://arxiv.org/pdf/2006.09882.pdf}
    \item semi-supervised representation learning (or meta representation learning)
\end{itemize}
